Semi-supervised Learning with Deep Generative Models for Asset Failure Prediction

This work presents a novel semi-supervised learning approach for data-driven modeling of asset failures when health status is only partially known in historical data. We combine a generative model parameterized by deep neural networks with non-linear embedding technique. It allows us to build prognostic models with the limited amount of health status information for the precise prediction of future asset reliability. The proposed method is evaluated on a publicly available dataset for remaining useful life (RUL) estimation, which shows significant improvement even when a fraction of the data with known health status is as sparse as 1% of the total. Our study suggests that the non-linear embedding based on a deep generative model can efficiently regularize a complex model with deep architectures while achieving high prediction accuracy that is far less sensitive to the availability of health status information.

==> 020background.tex <==
\subsection{Semi-supervised Learning}

Semi-supervised learning (SSL) aims to improve generalization on supervised tasks using unlabled data. In the semi-supervised learning framework, a given set of $N = L+U$ ($U >> L$ usually)  data can be divided into two parts: historical data $X_{l} = (x_{1},..,x_{l})$ for which corresponding labels $Y_{l} = (y_{1},..,y_{l})$ exist and $Xu = (x_{l+1},..,x_{l+u})$, for which corresponding labels do not exist. The goal of SSL is to improve prediction accuracy of a function learned from $(X_{l}, Y_{l})$, i.e., by taking into account the unlabeled data $X_{u}$. There are several assumptions that a number of SSL theories are based on. These are are smoothness, cluster, and manifold assumptions, each of which is related to the structure of the underlying distribution. While these assumptions are of great theoretical interest and may provide intuitions into SSL, we will not go into further details as our intention is not to uncover theoretical maximum performance gain that SSL approach can bring per se.

%It is generally known that several assumptions related to the structure of the underlying distribution must hold for SSL to improve prediction accuracy. These are are smoothness, cluster, and manifold assumptions. While each of the assumptions is of great theoretical interest and may provide intuitions into SSL, we will not go into further details as it is not the intention of this paper.
%It is generally known that SSL will not result in an improvement over supervised learning if certain assumptions related to the structure of the underlying distribution in data are not holds. It might even lower the prediction accuracy by misguiding the inference. These are smoothness, cluster, and manifold assumptions. While each of the assumptions is of great theoretical interest and may provide intuitions into SSL, we will not go into further details as it is not the scope of this paper.

%There are several assumptions such as smoothness, cluster, and manifold assumptions.
%While the (theoretical backgrounds) of such assumptions are of great interest/importance, we will not go into further It is not the scope of this work to go over the details of the assumptions as it is not the intention of the paper per se.

There exist numerous algorithms in semi-supervised learning [REF]. Probably the simplest of all is self-learing, which starts by building a base learner from small labeled samples. It then trains again with the labels obtained from the (best) prediction of the base learner, i.e., bootstrapping. This process is repeated until some condition is met. While It is known it often works well in practice [REF/NLP], it is prone to error because prediction mistake can be reinforced through repetitions. Performance gain is thus highly dependent on base learner's prediction confidence (accuracy) [REF].

Another popular set of approaches is based on well-studied probabilistic framework, i..e, generative models. Generative models try to model the conditional density $p(x|y)$ and make a prediction by inferring $p(y|x)$ from Bayes theorem. %finding the maximum likelihood estimate (MLE) of $\theta$ in $p(X,Y|\theta)$.
It is different from discriminative models in that generative models estimate the density of $x$ as an intermediate step. While there is different techniques such as Gaussian mixture (GMM), naive Bayes, and hidden markov models (HMM), our focus in on one of the generative models with deep architecture (DGM), known as variational autoencoder (VAE). We will give detailed explanation of VAE in the following section.

%1 Train f from (Xl,Yl)
%2 Predict on x ∈ Xu
%3 Add (x,f(x)) to labeled data
%4 Repeat

% 여기서 부터 어떻게 구성할 것인가?
% Embedding => Generative model
% Generatie model => Embedding

\subsection{Generative Models}

% DGM
% https://www.cs.cmu.edu/~rsalakhu/papers/annrev.pdf

Considering input variable $x$ and target variable $y$, a discriminative model focuses on $p(y|x)$, whereas a generative mode focuses on $P(x,y)$, which is often parameterized as $p(x|y)p(y)$ [REF-erhan]. Generative models have been recognized less prone to overfitting than discriminative models [REF - erhan, Ng andJordan]. Among different classes of generative models, those models with deep architectures composed of several layers of parameterized non-linear modules are called deep generative models (DGM). Approaches based on neural networks involve unsupervised embedding of the data either as a regularizer or as pre-trained layers for supervised learning [REF: KINGMA].

%Generative models can be used in numerous ways in SSL. In this article, we focus on
%that involve many layers of non-linear processing". %Deep belief networks and deep Boltzmann machines are

%"It has been recognized for some time that generative models are less prone to overfitting than discriminant ones" [REF-erhan]
%Considering input variable $\textbf{X}$ and target variable $\textbf{Y}$, a discriminant (discriminative) model focuses on $P(\textbf{Y}|\textbf{X})$, whereas a generative mode focuses on $P(\textbf{X},\textbf{Y})$, which is often parameterized as $P(\textbf{X}|\textbf{Y})P(\textbf{Y})$)[REF-erhan]


\subsection{Unsupervised Embedding}

Embedding is a procedure to map $x$ in the original space into a representation, where mapping is obtained from unsupervised (or semi-supervised) learning. Unsupervised embedding is used in SSL by exploiting information about $p(x)$ with a goal improve generalization of a supervised model (learner) [REF - ERHAN page 630]. Projecting into a representation found by unsupervised learning of Principal Component Analysis (PCA) is probably the most commonly used example of an embedding. However, PCA is limited in its capacity as it is linear model whilst many applications (dynamics) require non-linear modeling. The recent applications of DGM in unsupervised embedding have emerged as an exciting direction of SSL as they show state-of-the-art performance (shown promise) in various (unsupervised and) semi-supervised learning tasks.

%% Figure or Formula to help understanding?

% there are good theoretical and heuristic explanations why embedding help!
%.. to name a few. There exist various approaches to semi-supervised learning. As mentioned earlier, they are based on heuristic, generative models, and low-density separation. [more details regarding techniques? transductive , SVM, and so on].
%Probably the simplest of all is self-learing, which repeatedly uses a supervised learning algorithm (method). It starts by building a base-learner (weak-learner) from the (small) labeled samples. The unlabeled samples are labeled with the base-learner. The base-learner then is rebuilt by training the small labeled samples with the un-labeled samples with the labels from its own prediction. This process is repeated until some condition is met. This can be viewed as building bootstrapped models with label propagation. (This can be viewed as propagating labels.) While this approach can help improving the. . the performance is highly dependent on the confidence (accuracy) of base-learner and it is prone to in accuracy of base-learner get reinforced resulting in no improvement.
%\subsection{Recurrent Neural Networks}
%\subsubsection{Variational Autoencoder}







==> 100related.tex <==
{\bf Semi-supervised Learning} :
There exist numerous algorithms in semi-supervised learning [REF]. Probably the simplest of all is self-learing, which starts by building a base learner from small labeled samples. It then trains again with the labels obtained from the (best) prediction of the base learner, i.e., bootstrapping. This process is repeated until some condition is met. While It is known it often works well in practice [REF/NLP], it is prone to error because prediction mistake can be reinforced through repetitions. Performance gain is thus highly dependent on base learner's prediction confidence (accuracy) [REF].

Another popular set of approaches is based on well-studied probabilistic framework, i..e, generative models. Generative models try to model the conditional density $p(x|y)$ and make a prediction by inferring $p(y|x)$ from Bayes theorem. %finding the maximum likelihood estimate (MLE) of $\theta$ in $p(X,Y|\theta)$.
It is different from discriminative models in that generative models estimate the density of $x$ as an intermediate step. While there is different techniques such as Gaussian mixture (GMM), naive Bayes, and hidden markov models (HMM), our focus in on one of the generative models with deep architecture (DGM), known as variational autoencoder (VAE). We will give detailed explanation of VAE in the following section.


{\bf Generative Models }:
Considering input variable $x$ and target variable $y$, a discriminative model focuses on $p(y|x)$, whereas a generative mode focuses on $P(x,y)$, which is often parameterized as $p(x|y)p(y)$ [REF-erhan]. Generative models have been recognized less prone to overfitting than discriminative models [REF - erhan, Ng andJordan]. Among different classes of generative models, those models with deep architectures composed of several layers of parameterized non-linear modules are called deep generative models (DGM). Approaches based on neural networks involve unsupervised embedding of the data either as a regularizer or as pre-trained layers for supervised learning [REF: KINGMA].


{\bf Unsupervised Embedding}:
Embedding is a procedure to map $x$ in the original space into a representation, where mapping is obtained from unsupervised (or semi-supervised) learning. Unsupervised embedding is used in SSL by exploiting information about $p(x)$ with a goal improve generalization of a supervised model (learner) [REF - ERHAN page 630]. Projecting into a representation found by unsupervised learning of Principal Component Analysis (PCA) is probably the most commonly used example of an embedding. However, PCA is limited in its capacity as it is linear model whilst many applications (dynamics) require non-linear modeling. The recent applications of DGM in unsupervised embedding have emerged as an exciting direction of SSL as they show state-of-the-art performance (shown promise) in various (unsupervised and) semi-supervised learning tasks.

